Utility Assessment of Synthetic Data Generation Methods

Big data analysis poses the dual problem of privacy preservation and utility, i.e., how accurate data analyses remain after transforming original data in order to protect the privacy of the individuals that the data is about - and whether they are accurate enough to be meaningful. In this paper, we thus investigate across several datasets whether different methods of generating fully synthetic data vary in their utility a priori (when the specific analyses to be performed on the data are not known yet), how closely their results conform to analyses on original data a posteriori, and whether these two effects are correlated. We find some methods (decision-tree based) to perform better than others across the board, sizeable effects of some choices of imputation parameters (notably the number of released datasets), no correlation between broad utility metrics and analysis accuracy, and varying correlations for narrow metrics. We did get promising findings for classification tasks when using synthetic data for training machine learning models, which we consider worth exploring further also in terms of mitigating privacy attacks against ML models such as membership inference and model inversion.

==> effect_of_parameters.tex <==
\subsection{Comparison between Simple and Selective Imputation}
For the comparison between Simple and Selective imputation methods, we looked at the APO above 90\% using both the techniques alternatively for each synthesizer with Non-Proper imputation and $m = 10$. The reason behind choosing APO above 90\% is that it can show how well the synthesizers achieve 90\% goal and also can show what impact the Selective method has on the overall performance of the synthesizers. We used 20 regression tests for Polish and 24 for both Adult and Avila. 

Table \ref{tab:simple_selective_short} shows for the all three datasets the average and the ratio of how many regression fits were better for Simple and Selective respectively for each synthesizer. We can see that for all of the three datasets for majority of the synthesizers Simple works better than Selective. When we look at the individual regression fits, some of the synthesizer combinations and some regression fits perform better with Selective than Simple but it is not very common. One interesting thing to note here is that even though the difference between Simple and Selective varies a lot for the different synthesizers, their accuracy for Simple was pretty close.

For Polish, the Simple method was better regardless of the synthesizer combinations. However, for Adult and Avila, we see that few synthesizer combinations performed better with Selective imputation. For Adult, CAP and CAC with Selective performed slightly better than Simple. Nonetheless, SAP with imputation order largest categorical variable last (PL) achieved a significant improvement with Selective. When we look at the individual regression fits we see that, for most of the synthesizer combinations, only a couple of regression fits are responsible for dragging the average down. The Selective PL is able to handle those regression fits better than Simple and that is the why it achieves higher score. For Avila, except SAP with opposite imputation order (PO), Simple performed better than Selective for all the other synthesizer combinations.  
% \vspace{0.5em}
% \\
% \fcolorbox{black}{lightgray}{
% \begin{minipage}{24em}
% \textbf{Summary:} Based on our experiments it is evident that Simple is preferred more for general purpose usage since it performs better for most of the synthesizer combinations for all three datasets. For Selective imputation the knowledge about the datasets including which relationship between variables are important is necessary which is not the case for Simple making it an easier choice. However, if the dataset is too large with a lot variables then Simple may not be feasible and Selective would be the only choice. For the datasets we have tested, it is possible to use both Simple and Selective imputation. One thing we  noticed that the time difference between Simple and Selective is not substantial and surprisingly for CAP Selective was on an average slower than Simple. Thus, for general purpose usage and for datasets that are not too large Simple is a better choice whereas for specific use cases and larger datasets with a lot of variables Selective is the way to go.     
% \end{minipage}
% }
% \\
\input{figures_tables/tb_simple_selective_short}
%Table APO over 90\% comparison between the Simple method and the Selective method with m = 10 and type 1 variance for synthesizers: SAP (P), Cart (D), CAP (CP) and CAC (CC).
\subsection{Comparison between Proper and Non-proper Imputation}
To compare proper and non-proper imputation, we ran the experiments for each synthesizer with both the methods individually. In the figures Proper imputations are symbolized with $T$ suffix and without $T$ suffix symbolize Non-Proper versions. For instance, $D$ symbolizes Non-Proper version of decision tree and $DT$ symbolizes the Proper version of the same synthesizer.   

We will now look at the result with APO above $90$ (Figure \ref{fig:apo_90_t1}). The first thing to notice is that for all three datasets for lower $m$ (e.g. $m = \{1,2,3\}$ Proper methods perform far worse than Non-Proper methods regardless of synthesizer combinations. The reason for Proper working poorly for small $m$ is that it is essentially an imputation from a random sample of the original data which means that the imputation is done from a dataset that is not the original dataset. So when results from mean point estimation, KL-divergence or regression fits are compared with the original they are worse since the sample does not represent the original dataset well.
% \vspace{0.5em}
% \\
% \fcolorbox{black}{lightgray}{
% \begin{minipage}{24em}
% \textbf{Summary:} For higher $m$, in majority cases Proper method either falls behind with close margin or performs worse than the Non-Proper method with few exceptions (e.g. Cart for Adult). Proper ones are on an average worse than the Non-Proper synthesizers and stay behind even when $m$ increases for most of the synthesizers. Thus, Proper should not be used if one is not going to release many dataset and instead use Non-Proper. With large $m$ one should most likely use Non-Proper here as well but since Proper could be better or worse, one should test which one works the best.
% \end{minipage}
% }
% \\
\subsection{Effect of Number of Datasets}
To see the effects number of datasets on the performance of the synthesizers, we experimented by varying the number of datasets. In the figures and tables $m$ represents the number of datasets.

From mean point estimation with Raab combining rule (Table \ref{tab:mpe_type_1}), we see that for all three datasets lower $m$ fails to achieve APO over 90\% for all synthesizer combinations. For instance, it required  at least $m = 3$ for most of the synthesizers that eventually achieved APO over 90 to either achieve it or reach very close it for Polish and Adult and for Avila the requirement is even higher. 

From average CI overlap of regression fit with Raab combining rule (Fig \ref{fig:rf_t1}), we see that for all three datasets and most of the synthesizer combinations the overlap plateaus very early and does not increase much with the increase in number of datasets. For instance. in the case of Polish dataset we see that there is a steady increase in CI overlap with the increase of $m$. For all three datasets, we see that the return gradually diminishes with the largest increases being below 10 to 20 datasets and the overlaps above only increasing in small amounts. Moreover, in the case of Adult and Avila, the average CI overlap even drops for many of the synthesizers (e.g. Cart (D) for Adult and SAP with opposite order (PO) for Avila) with the increase of $m$. 

From the results of mean point estimation and average CI overlap of regression fits, it seems that lower $m$ values (i.e. $m = \{1, 2\}$) do not perform very poorly compared to the higher values. However, when we look at the APO above 90\% of regression coefficients (Fig \ref{fig:apo_90_t1}) for all three datasets we can see that lower $m$ (e.g. $m = \{1, 2\}$ is far worse than higher $m$. Moreover, the accuracy of the synthesizers also increase steadily for larger $m$ values above $5$. 
% \vspace{0.5em}
% \\
% \fcolorbox{black}{lightgray}{
% \begin{minipage}{24em}
% \textbf{Summary:} From the experiments it is very evident that releasing multiple datasets is better than releasing just one synthetic dataset. One can argue that by releasing higher number datasets such as $m > 100$, it is possible to get better accuracy. However, there can be two potential problems of releasing such high number of datasets which are size and privacy. If the original dataset is already too large then the computational complexity may not be feasible to allow the generation of such large number of datasets. Similarly, in terms of privacy, the more you release data the more the privacy risk. Thus, when choosing the number of dataset we need to find a correct balance between, utility, privacy and computational complexity depending on the specific use case scenarios of the synthetic data. 
% \end{minipage}
% }
% \\
\subsection{Effect of Imputation Order}
For analyzing the effect of imputation order we experimented with different orders for each synthesizers. For Polish and Avila we use original ordering (no suffix), the opposite ordering (O) and our own ordering (V). Our own ordering for Polish is the order that we think makes the most sense with regards to preserving relationships between variables and for Avila it is just moving the only categorical variable to the middle of the original order. For Adult, we use the original order (no-suffix), the largest categorical variable first (H), and the largest categorical variable last (L) ordering. In figures and tables the suffix mentioned above symbolizes the ordering. For instance, $P$ symbolizes SAP with original ordering, $PO$ symbolizes SAP with opposite ordering, and  $POT$ symbolizes SAP with opposite ordering and Proper imputation. 

For Polish dataset (Fig \ref{fig:polish_apo_90_t1}), original ordering id best overall whereas the opposite ordering performed worst. The own ordering for Polish performed slightly worse than the original ordering. In the case of Adult (Fig \ref{fig:adult_apo_90_t1}), largest categorical variable last imputation with Cart (DL) performed better than a lot of other synthesizers. Lastly for Avila (Fig \ref{fig:avila_apo_90_t1}), own ordering with Cart (DV) performed better that CAC which was not the case for Polish or Adult. CAC in this case just Cart but with a different imputation order. 
% \vspace{0.5em}
% \\
% \fcolorbox{black}{lightgray}{
% \begin{minipage}{24em}
% \textbf{Summary:} The imputation order  can have a big impact on the result where one order can differ from the other by even $20$ percentage points (Cart in Figure \ref{fig:rf_t1}). However, it is not possible to separate the effect of the choice of order and the preserved relationships on the utility. This makes it hard to draw any conclusions on whether it is the order that has such a huge effect on utility or if it is the difference in relationships used for the imputation or if it is a mixture of both. Thus, testing with different imputation orders with different synthesizers can help to find the best combination.  
% \end{minipage}
% }
% \\
\begin{figure*}[htbp]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures_tables/fig_polish_gen_time_simp.pdf}
  \caption{Polish Dataset - Simple}
  \label{fig:polish_gen_time_simp}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures_tables/fig_adult_gen_time_simp.pdf}
  \caption{Adult Dataset - Simple}
  \label{fig:adult_gen_time_simp}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures_tables/fig_avila_gen_time_simp.pdf}
  \caption{Avila Dataset - Simple}
  \label{fig:avila_gen_time_simp}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures_tables/fig_polish_gen_time_sel.pdf}
  \caption{Polish Dataset - Selective}
  \label{fig:polish_gen_time_sel}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures_tables/fig_adult_gen_time_sel.pdf}
  \caption{Adult Dataset - Selective}
  \label{fig:adult_gen_time_sel}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures_tables/fig_avila_gen_time_sel.pdf}
  \caption{Avila Dataset - Selective}
  \label{fig:avila_gen_time_sel}
\end{subfigure}
\caption{APO above 90\% over the generation time for 100 datasets for synthesizers: SAP (P), Cart (D), CAP (CP) and CAC (CC).}
\label{fig:gen_time}
\end{figure*}

\subsection{Generation Time}
For generation time, we plot APO above $90$\% with the time it took to generate $100$ datasets for each synthesizer combination for both the Simple and the Selective methodology in Figures \ref{fig:gen_time}. 

For Polish (Figure \ref{fig:polish_gen_time_simp}), we can see that the fastest option is CAC, then Cart, followed by SAP and the longest was CAP. In terms of accuracy, based on average CI overlap (Figure \ref{fig:polish_rf_t1}) and APO above 90\% (Figure \ref{fig:polish_apo_90_t1}) for regression fits, CAC in the best synthesizer for polish and in terms of generation time it is also the fastest. Nonetheless, one interesting finding to note here is that, as we saw previously in terms of accuracy CAP and Cart are very similar, but the generation time difference is far larger between the two. Since Cart is not far behind in terms of accuracy and out performs CAP in terms of generation time for it is hard to justify using CAP over Cart for polish. We can also see that there is no huge difference between the selection of Proper and Non-Proper for the generation time for any synthesizer combinations. While Selective (Figure \ref{fig:polish_gen_time_sel}) is faster for most (CAP being a strange exception), it is not too much faster here for Cart and CAC though SAP and CAP see real improvements. The different imputation orders for Cart and SAP do not seem to have as much impact as the selection of synthesizer.

For Adult (Figure \ref{fig:adult_gen_time_simp}), we can see that Cart is the fastest, even faster than CAC as well. CAP is third slowest synthesizer but is still faster than all the SAP synthesizer combinations. Proper and Non-Proper showed some real difference for Cart but even more for SAP here when compared with CAC and CAP for Polish. The reason for this is unclear but the large difference for SAP could be because of the small sample size due to the long imputation time for SAP and since those large difference were true both for Selective (Figure \ref{fig:adult_gen_time_sel}) as well it might be a real phenomenon. The reason why this could be happening is that Proper SAP can be faster than Non-Proper to converge while generating the imputation models. Selective (Figure \ref{fig:adult_gen_time_sel}) was also faster for all of them except CPT. The choice of imputation order had a huge effect on the generation time for SAP with the slowest taking 10 times as long as the fastest. Cart saw some pretty significant difference as well with the slowest taking about twice as long to generate as the fastest.  Even if Cart was faster one would probably still favour CAC or maybe even CAP for the increased utility over Cart. One would most likely not use SAP even if Selective PL performed pretty well being more than a $100$ times slower than Cart or CAC.

Finally, for Avila (Figure \ref{fig:avila_gen_time_simp}), Cart, CAC and SAP were a lot closer together than previously but SAP still varied a lot depending on which order was used for the imputation while Cart was more consistent. PO and POT was a lot faster than the other synthesizers because the numerical variable imputations are much faster for SAP than categorical and since the single categorical variable was in the beginning, it was turned into a sample. CAP however is the slowest for Avila taking about 40 times as long as Cart. Proper and Non-Proper were relatively close again. Selective (Figure \ref{fig:avila_gen_time_sel}) did see moderate improvements in generation time for all synthesizers, even for CAP as well. While PO was much faster than the other synthesizers and while Selective was also faster than Simple, one would never pick any of those two though since the performance was so much worse than Cart and CAC making those two the only real option here.
% \vspace{0.5em}
% \\
% \fcolorbox{black}{lightgray}{
% \begin{minipage}{24em}
% \textbf{Summary:} In terms of generation time, CAC and Cart are among the top three fastest performing synthesizers for all three datasets. Even though in terms of accuracy CAP is close to Cart and CAC, it is much slower than the two for all three datasets. In case of Simple and Selective, though Selective was faster overall, the difference between them was not significant. Proper and Non-proper also do not show any significant difference between them in terms of generation time. For Avila, SAP was fastest however, it performs poorly in terms of accuracy. So, there in no point of choosing SAP for Avila. 
% \end{minipage}
% }
% \\
%\subsubsection{Privacy Comparison}
%\subsubsection{Generation Time Comparison}

==> figures_tables/tb_simple_selective.tex <==
\begin{table*}[!htbp]
\caption{APO over $90$\% comparison between the Simple method and the Selective method with $m = 10$ and type 1 variance for synthesizers: SAP (P), Cart (D), CAP (CP) and CAC (CC)}
\label{tab:simple_selective}
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r|rrrrrrrrrrrrrrrr}
  \hline
  fit & P & PSe & D & DSe & PO & POSe & DO & DOSe & PV & PVSe & DV & DVSe & CP & CPSe & CC & CCSe \\ 
  \hline
  1 & 0.01 & 0.00 & 0.43 & 0.63 & 0.03 & 0.11 & 0.05 & 0.00 & 0.00 & 0.00 & 0.71 & 0.71 & 0.31 & 0.36 & 0.34 & 0.63 \\ 
  2 & 0.00 & 0.00 & 0.60 & 0.64 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.68 & 0.67 & 0.62 & 0.47 & 0.40 & 0.54 \\ 
  3 & 0.45 & 0.09 & 0.34 & 0.16 & 0.77 & 0.15 & 0.07 & 0.03 & 0.48 & 0.09 & 0.37 & 0.15 & 0.43 & 0.14 & 0.39 & 0.15 \\ 
  4 & 0.67 & 0.20 & 0.48 & 0.31 & 0.52 & 0.08 & 0.04 & 0.09 & 0.57 & 0.14 & 0.33 & 0.36 & 0.63 & 0.42 & 0.40 & 0.34 \\ 
  5 & 0.13 & 0.29 & 0.41 & 0.21 & 0.68 & 0.18 & 0.10 & 0.00 & 0.25 & 0.32 & 0.23 & 0.22 & 0.49 & 0.48 & 0.57 & 0.53 \\ 
  6 & 0.55 & 0.42 & 0.17 & 0.22 & 0.70 & 0.07 & 0.04 & 0.05 & 0.56 & 0.28 & 0.10 & 0.08 & 0.64 & 0.59 & 0.67 & 0.67 \\ 
  7 & 0.05 & 0.04 & 0.23 & 0.00 & 0.03 & 0.00 & 0.35 & 0.06 & 0.03 & 0.06 & 0.51 & 0.00 & 0.80 & 0.69 & 0.80 & 0.62 \\ 
  8 & 0.34 & 0.26 & 0.63 & 0.45 & 0.46 & 0.13 & 0.26 & 0.14 & 0.34 & 0.27 & 0.36 & 0.37 & 0.67 & 0.78 & 0.76 & 0.77 \\ 
  9 & 0.68 & 0.50 & 0.36 & 0.31 & 0.55 & 0.41 & 0.31 & 0.28 & 0.68 & 0.50 & 0.34 & 0.31 & 0.65 & 0.66 & 0.64 & 0.53 \\ 
  10 & 0.56 & 0.22 & 0.48 & 0.16 & 0.53 & 0.35 & 0.01 & 0.38 & 0.56 & 0.24 & 0.27 & 0.24 & 0.38 & 0.39 & 0.77 & 0.77 \\ 
  11 & 0.41 & 0.65 & 0.66 & 0.45 & 0.48 & 0.34 & 0.20 & 0.59 & 0.38 & 0.59 & 0.50 & 0.48 & 0.47 & 0.73 & 0.53 & 0.49 \\ 
  12 & 0.58 & 0.21 & 0.29 & 0.15 & 0.23 & 0.29 & 0.27 & 0.12 & 0.73 & 0.34 & 0.34 & 0.29 & 0.34 & 0.19 & 0.74 & 0.24 \\ 
  13 & 0.00 & 0.00 & 0.65 & 0.44 & 0.00 & 0.13 & 0.28 & 0.33 & 0.00 & 0.00 & 0.55 & 0.44 & 0.26 & 0.19 & 0.57 & 0.74 \\ 
  14 & 0.07 & 0.08 & 0.75 & 0.39 & 0.00 & 0.00 & 0.53 & 0.06 & 0.09 & 0.08 & 0.44 & 0.27 & 0.19 & 0.16 & 0.66 & 0.69 \\ 
  15 & 0.24 & 0.25 & 0.83 & 0.41 & 0.14 & 0.11 & 0.43 & 0.16 & 0.23 & 0.25 & 0.59 & 0.32 & 0.54 & 0.26 & 0.84 & 0.75 \\ 
  16 & 0.70 & 0.65 & 0.41 & 0.35 & 0.20 & 0.11 & 0.29 & 0.38 & 0.68 & 0.64 & 0.50 & 0.24 & 0.43 & 0.52 & 0.49 & 0.36 \\ 
  17 & 0.62 & 0.32 & 0.49 & 0.31 & 0.38 & 0.30 & 0.35 & 0.34 & 0.57 & 0.30 & 0.38 & 0.29 & 0.64 & 0.23 & 0.47 & 0.25 \\ 
  18 & 0.56 & 0.00 & 0.74 & 0.00 & 0.13 & 0.00 & 0.04 & 0.00 & 0.56 & 0.00 & 0.77 & 0.00 & 0.30 & 0.00 & 0.64 & 0.00 \\ 
  19 & 0.56 & 0.08 & 0.47 & 0.08 & 0.30 & 0.10 & 0.46 & 0.01 & 0.40 & 0.06 & 0.54 & 0.08 & 0.49 & 0.08 & 0.39 & 0.07 \\ 
  20 & 0.31 & 0.12 & 0.51 & 0.32 & 0.48 & 0.42 & 0.17 & 0.28 & 0.63 & 0.11 & 0.57 & 0.25 & 0.60 & 0.65 & 0.44 & 0.41 \\ 
  \hline
  Average & 0.38 & 0.22 & 0.50 & 0.30 & 0.33 & 0.16 & 0.21 & 0.16 & 0.39 & 0.21 & 0.45 & 0.29 & 0.49 & 0.40 & 0.58 & 0.48 \\ 
  \hline
  Ratio & 0.78 & 0.22 & 0.85 & 0.15 & 0.83 & 0.17 & 0.63 & 0.37 & 0.76 & 0.24 & 0.90 & 0.10 & 0.65 & 0.35 & 0.75 & 0.25 \\  
  \hline
\end{tabular}%
}
\caption{Polish Dataset}
\label{tab:polish_simple_selective}
\end{subtable}%
\hfill
\begin{subtable}{0.48\textwidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r|rrrrrrrrrrrrrrrr}
  \hline
  fit & P & PSe & D & DSe & PH & PHSe & DH & DHSe & PL & PLSe & DL & DLSe & CP & CPSe & CC & CCSe \\ 
  \hline
  1 & 0.37 & 0.30 & 0.13 & 0.09 & 0.66 & 0.54 & 0.13 & 0.07 & 0.45 & 0.76 & 0.18 & 0.16 & 0.78 & 0.78 & 0.78 & 0.78 \\ 
  2 & 0.51 & 0.12 & 0.23 & 0.06 & 0.54 & 0.11 & 0.19 & 0.04 & 0.43 & 0.55 & 0.55 & 0.51 & 0.70 & 0.71 & 0.72 & 0.75 \\ 
  3 & 0.44 & 0.42 & 0.48 & 0.26 & 0.53 & 0.45 & 0.13 & 0.21 & 0.55 & 0.46 & 0.34 & 0.16 & 0.79 & 0.78 & 0.76 & 0.75 \\ 
  4 & 0.17 & 0.17 & 0.22 & 0.14 & 0.26 & 0.19 & 0.55 & 0.53 & 0.41 & 0.54 & 0.41 & 0.61 & 0.28 & 0.28 & 0.28 & 0.27 \\ 
  5 & 0.40 & 0.26 & 0.12 & 0.01 & 0.51 & 0.35 & 0.01 & 0.07 & 0.38 & 0.44 & 0.39 & 0.16 & 0.76 & 0.71 & 0.76 & 0.71 \\ 
  6 & 0.53 & 0.61 & 0.19 & 0.15 & 0.40 & 0.42 & 0.22 & 0.09 & 0.43 & 0.49 & 0.22 & 0.27 & 0.44 & 0.54 & 0.48 & 0.51 \\ 
  7 & 0.49 & 0.07 & 0.31 & 0.06 & 0.40 & 0.08 & 0.24 & 0.05 & 0.51 & 0.49 & 0.53 & 0.51 & 0.64 & 0.68 & 0.73 & 0.69 \\ 
  8 & 0.18 & 0.00 & 0.20 & 0.18 & 0.37 & 0.04 & 0.27 & 0.16 & 0.03 & 0.01 & 0.05 & 0.11 & 0.29 & 0.36 & 0.35 & 0.36 \\ 
  9 & 0.27 & 0.15 & 0.16 & 0.08 & 0.34 & 0.10 & 0.09 & 0.08 & 0.29 & 0.25 & 0.12 & 0.11 & 0.35 & 0.33 & 0.35 & 0.29 \\ 
  10 & 0.24 & 0.00 & 0.12 & 0.00 & 0.30 & 0.00 & 0.01 & 0.00 & 0.56 & 0.23 & 0.75 & 0.09 & 0.79 & 0.79 & 0.80 & 0.79 \\ 
  11 & 0.22 & 0.00 & 0.06 & 0.00 & 0.26 & 0.00 & 0.00 & 0.00 & 0.14 & 0.10 & 0.75 & 0.00 & 0.77 & 0.78 & 0.81 & 0.78 \\ 
  12 & 0.61 & 0.64 & 0.23 & 0.12 & 0.64 & 0.57 & 0.07 & 0.11 & 0.60 & 0.38 & 0.17 & 0.10 & 0.80 & 0.82 & 0.81 & 0.80 \\ 
  13 & 0.62 & 0.43 & 0.16 & 0.10 & 0.49 & 0.44 & 0.12 & 0.09 & 0.35 & 0.54 & 0.19 & 0.29 & 0.65 & 0.64 & 0.66 & 0.62 \\ 
  14 & 0.00 & 0.00 & 0.32 & 0.12 & 0.00 & 0.00 & 0.19 & 0.14 & 0.00 & 0.14 & 0.16 & 0.14 & 0.17 & 0.27 & 0.20 & 0.26 \\ 
  15 & 0.00 & 0.00 & 0.23 & 0.10 & 0.00 & 0.00 & 0.25 & 0.16 & 0.00 & 0.14 & 0.14 & 0.11 & 0.17 & 0.28 & 0.21 & 0.35 \\ 
  16 & 0.00 & 0.00 & 0.33 & 0.13 & 0.00 & 0.00 & 0.19 & 0.15 & 0.00 & 0.19 & 0.19 & 0.17 & 0.19 & 0.27 & 0.21 & 0.24 \\ 
  17 & 0.00 & 0.00 & 0.27 & 0.17 & 0.00 & 0.00 & 0.27 & 0.25 & 0.00 & 0.21 & 0.15 & 0.13 & 0.21 & 0.21 & 0.21 & 0.24 \\ 
  18 & 0.00 & 0.00 & 0.47 & 0.58 & 0.00 & 0.00 & 0.52 & 0.53 & 0.00 & 0.53 & 0.28 & 0.27 & 0.41 & 0.74 & 0.60 & 0.63 \\ 
  19 & 0.00 & 0.00 & 0.30 & 0.37 & 0.00 & 0.00 & 0.36 & 0.43 & 0.00 & 0.48 & 0.29 & 0.22 & 0.53 & 0.37 & 0.30 & 0.71 \\ 
  20 & 0.00 & 0.00 & 0.45 & 0.51 & 0.00 & 0.00 & 0.47 & 0.51 & 0.00 & 0.50 & 0.29 & 0.30 & 0.47 & 0.70 & 0.56 & 0.61 \\ 
  21 & 0.00 & 0.00 & 0.34 & 0.47 & 0.00 & 0.00 & 0.37 & 0.49 & 0.00 & 0.63 & 0.31 & 0.22 & 0.56 & 0.37 & 0.32 & 0.58 \\ 
  22 & 0.56 & 0.34 & 0.42 & 0.31 & 0.56 & 0.29 & 0.40 & 0.23 & 0.52 & 0.53 & 0.49 & 0.43 & 0.53 & 0.53 & 0.33 & 0.39 \\ 
  23 & 0.61 & 0.50 & 0.20 & 0.21 & 0.59 & 0.44 & 0.29 & 0.24 & 0.35 & 0.39 & 0.28 & 0.24 & 0.58 & 0.52 & 0.46 & 0.52 \\ 
  24 & 0.63 & 0.69 & 0.49 & 0.47 & 0.66 & 0.73 & 0.44 & 0.40 & 0.18 & 0.48 & 0.18 & 0.28 & 0.50 & 0.63 & 0.58 & 0.56 \\ 
  \hline
  Average & 0.29 & 0.20 & 0.27 & 0.20 & 0.31 & 0.20 & 0.24 & 0.21 & 0.26 & 0.39 & 0.31 & 0.23 & 0.51 & 0.55 & 0.51 & 0.55 \\ 
  \hline
  Ratio & 0.81 & 0.19 & 0.79 & 0.21 & 0.88 & 0.12 & 0.70 & 0.30 & 0.29 & 0.71 & 0.75 & 0.25 & 0.30 & 0.70 & 0.46 & 0.54 \\ 
  \hline
\end{tabular}%
}
\caption{Adult Dataset}
\label{tab:adult_simple_selective}
\end{subtable}%
\hspace{\fill} 
\begin{subtable}{0.48\textwidth}
\flushright
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r|rrrrrrrrrrrrrrrr}
  \hline
  fit & P & PSe & D & DSe & PO & POSe & DO & DOSe & PV & PVSe & DV & DVSe & CP & CPSe & CC & CCSe \\ 
  \hline
  1 & 0.07 & 0.14 & 0.11 & 0.00 & 0.01 & 0.11 & 0.07 & 0.08 & 0.08 & 0.02 & 0.18 & 0.00 & 0.23 & 0.00 & 0.18 & 0.04 \\ 
  2 & 0.05 & 0.04 & 0.01 & 0.01 & 0.14 & 0.12 & 0.24 & 0.17 & 0.26 & 0.17 & 0.19 & 0.04 & 0.33 & 0.21 & 0.19 & 0.15 \\ 
  3 & 0.26 & 0.25 & 0.27 & 0.00 & 0.06 & 0.14 & 0.14 & 0.16 & 0.37 & 0.36 & 0.42 & 0.07 & 0.37 & 0.14 & 0.43 & 0.12 \\ 
  4 & 0.17 & 0.15 & 0.26 & 0.13 & 0.13 & 0.21 & 0.36 & 0.25 & 0.39 & 0.24 & 0.28 & 0.10 & 0.41 & 0.19 & 0.33 & 0.13 \\ 
  5 & 0.09 & 0.10 & 0.11 & 0.00 & 0.04 & 0.14 & 0.16 & 0.06 & 0.03 & 0.07 & 0.22 & 0.11 & 0.13 & 0.00 & 0.20 & 0.05 \\ 
  6 & 0.15 & 0.19 & 0.13 & 0.03 & 0.10 & 0.08 & 0.34 & 0.11 & 0.18 & 0.14 & 0.36 & 0.12 & 0.40 & 0.12 & 0.48 & 0.26 \\ 
  7 & 0.16 & 0.22 & 0.24 & 0.00 & 0.11 & 0.17 & 0.24 & 0.24 & 0.19 & 0.23 & 0.29 & 0.02 & 0.20 & 0.32 & 0.25 & 0.37 \\ 
  8 & 0.09 & 0.03 & 0.11 & 0.00 & 0.06 & 0.03 & 0.12 & 0.09 & 0.15 & 0.12 & 0.09 & 0.05 & 0.08 & 0.06 & 0.13 & 0.15 \\ 
  9 & 0.00 & 0.00 & 0.06 & 0.10 & 0.10 & 0.06 & 0.04 & 0.05 & 0.01 & 0.01 & 0.25 & 0.04 & 0.02 & 0.01 & 0.19 & 0.02 \\ 
  10 & 0.06 & 0.01 & 0.11 & 0.09 & 0.11 & 0.12 & 0.20 & 0.10 & 0.03 & 0.01 & 0.20 & 0.10 & 0.20 & 0.14 & 0.48 & 0.13 \\ 
  11 & 0.08 & 0.06 & 0.03 & 0.00 & 0.00 & 0.07 & 0.10 & 0.12 & 0.00 & 0.02 & 0.15 & 0.10 & 0.14 & 0.06 & 0.25 & 0.08 \\ 
  12 & 0.00 & 0.00 & 0.11 & 0.03 & 0.11 & 0.18 & 0.26 & 0.06 & 0.09 & 0.04 & 0.38 & 0.06 & 0.12 & 0.05 & 0.27 & 0.17 \\ 
  13 & 0.15 & 0.03 & 0.39 & 0.00 & 0.30 & 0.28 & 0.16 & 0.34 & 0.17 & 0.18 & 0.43 & 0.00 & 0.60 & 0.40 & 0.38 & 0.38 \\ 
  14 & 0.11 & 0.07 & 0.00 & 0.00 & 0.02 & 0.07 & 0.17 & 0.00 & 0.11 & 0.00 & 0.06 & 0.07 & 0.22 & 0.00 & 0.08 & 0.01 \\ 
  15 & 0.00 & 0.16 & 0.06 & 0.00 & 0.00 & 0.00 & 0.23 & 0.00 & 0.22 & 0.09 & 0.28 & 0.00 & 0.16 & 0.00 & 0.14 & 0.00 \\ 
  16 & 0.14 & 0.00 & 0.29 & 0.16 & 0.10 & 0.04 & 0.51 & 0.48 & 0.06 & 0.27 & 0.50 & 0.15 & 0.32 & 0.08 & 0.34 & 0.38 \\ 
  17 & 0.12 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.16 & 0.00 & 0.03 & 0.01 \\ 
  18 & 0.12 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.16 & 0.00 & 0.03 & 0.01 \\ 
  19 & 0.01 & 0.00 & 0.21 & 0.01 & 0.12 & 0.12 & 0.22 & 0.30 & 0.00 & 0.00 & 0.36 & 0.15 & 0.18 & 0.06 & 0.43 & 0.22 \\ 
  20 & 0.14 & 0.09 & 0.19 & 0.11 & 0.00 & 0.00 & 0.35 & 0.00 & 0.01 & 0.03 & 0.16 & 0.00 & 0.23 & 0.01 & 0.20 & 0.17 \\ 
  21 & 0.00 & 0.02 & 0.15 & 0.19 & 0.00 & 0.00 & 0.05 & 0.01 & 0.04 & 0.05 & 0.20 & 0.12 & 0.17 & 0.02 & 0.07 & 0.20 \\ 
  22 & 0.05 & 0.04 & 0.25 & 0.02 & 0.01 & 0.00 & 0.18 & 0.37 & 0.00 & 0.01 & 0.41 & 0.10 & 0.44 & 0.53 & 0.49 & 0.52 \\ 
  23 & 0.23 & 0.18 & 0.20 & 0.07 & 0.03 & 0.03 & 0.04 & 0.18 & 0.29 & 0.21 & 0.21 & 0.16 & 0.18 & 0.01 & 0.20 & 0.23 \\ 
  24 & 0.03 & 0.11 & 0.08 & 0.07 & 0.00 & 0.00 & 0.09 & 0.12 & 0.03 & 0.06 & 0.10 & 0.05 & 0.04 & 0.08 & 0.11 & 0.05 \\ 
  \hline
  Average & 0.10 & 0.08 & 0.14 & 0.04 & 0.06 & 0.08 & 0.18 & 0.14 & 0.11 & 0.10 & 0.24 & 0.07 & 0.23 & 0.10 & 0.24 & 0.16 \\ 
  \hline
  Ratio & 0.68 & 0.32 & 0.91 & 0.09 & 0.37 & 0.63 & 0.61 & 0.39 & 0.58 & 0.42 & 0.96 & 0.04 & 0.88 & 0.12 & 0.74 & 0.26 \\ 
  \hline
\end{tabular}%
}
\caption{Avila Dataset}
\label{tab:avila_simple_selective}
\end{subtable}
\end{table*}

==> figures_tables/tb_synthesizer_MPE_t2.tex <==
\begin{table*}[!htbp]
\caption{APO over $90$\% for all mean point estimators with type 2 variance for synthesizers: Sample (S), SAP (P), Cart (D), CAP (CP) and CAC (CC)}
\label{tab:mpe_type_2}
\begin{subtable}{.3\linewidth}
\centering
\begin{tabular}{r|rrrrr}
\hline
\textbf{m} & \textbf{S} & \textbf{P} & \textbf{D} & \textbf{CP} & \textbf{CC} \\ \hline
2 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
3 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
5 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
10 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
20 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
50 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
100 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\ \hline
\end{tabular}
\caption{Polish Dataset}
\label{tab:polish_mpe_type_2}
\end{subtable}%
\hfill
\begin{subtable}{.3\linewidth}
\centering
\begin{tabular}{r|rrrrr}
\hline
\textbf{m} & \textbf{S} & \textbf{P} & \textbf{D} & \textbf{CP} & \textbf{CC} \\ \hline
2 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
3 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
5 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
10 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
20 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
50 & 1.00 & 0.50 & 1.00 & 1.00 & 1.00 \\
100 & 1.00 & - & 1.00 & 1.00 & 1.00 \\ \hline
\end{tabular}%
\caption{Adult Dataset}
\label{tab:adult_mpe_type_2}
\end{subtable}%
\hfill
\begin{subtable}{.3\linewidth}
\centering
\begin{tabular}{r|rrrrr}
\hline
\textbf{m} & \textbf{S} & \textbf{P} & \textbf{D} & \textbf{CP} & \textbf{CC} \\ \hline
2 & 0.93 & 0.84 & 0.93 & 0.85 & 0.93 \\
3 & 0.95 & 0.84 & 0.95 & 0.87 & 0.95 \\
5 & 0.96 & 0.85 & 0.96 & 0.86 & 0.96 \\
10 & 0.98 & 0.87 & 0.98 & 0.87 & 0.98 \\
20 & 1.00 & 0.88 & 0.99 & 0.87 & 1.00 \\
50 & 1.00 & 0.89 & 1.00 & 0.88 & 1.00 \\
100 & 1.00 & 0.90 & 1.00 & 0.89 & 1.00 \\ \hline
\end{tabular}
\caption{Avila Dataset}
\label{tab:avila_mpe_type_2}
\end{subtable}
\end{table*}

==> figures_tables/tb_synthesizers_kl_divergence.tex <==
\begin{table*}[!htbp]
\tiny
\caption{KL-Divergence score normalized over S's KL-Divergence score for synthesizers: Sample (S), SAP (P), Cart (D), CAP (CP) and CAC (CC).}
\label{tab:kl_dv_syn}
\resizebox{\textwidth}{!}{
\begin{subtable}{0.36\linewidth}
\centering
\begin{tabular}{r|rrrrr}
\hline
\textbf{Variable} & \textbf{S} & \textbf{P} & \textbf{D} & \textbf{CP} & \textbf{CC} \\ \hline
sex & 1.00 & 1.09 & 1.11 & 1.10 & 1.00 \\
age & 1.00 & 1.02 & 1.00 & 1.04 & 1.00 \\
edu & 1.00 & 1.00 & 0.96 & 1.01 & 0.96 \\
marital & 1.00 & 1.04 & 1.01 & 0.99 & 1.02 \\
income & 1.00 & 1.14 & 1.06 & 1.12 & 1.01 \\
ls & 1.00 & 1.04 & 1.06 & 1.04 & 1.02 \\
trust & 1.00 & 1.12 & 1.08 & 1.09 & 1.11 \\
nofriend & 1.00 & 1.15 & 1.07 & 1.11 & 1.06 \\
smoke & 1.00 & 1.03 & 1.36 & 1.01 & 0.95 \\
alcabuse & 1.00 & 1.29 & 1.08 & 1.04 & 1.05 \\
wkabint & 1.00 & 1.72 & 0.96 & 1.06 & 1.08 \\
englang & 1.00 & 1.59 & 0.99 & 0.97 & 0.99 \\
height & 1.00 & 1.65 & 1.06 & 1.14 & 1.05 \\
weight & 1.00 & 1.07 & 1.06 & 1.21 & 1.08 \\ \hline
Average & 1.00 & 1.21 & 1.06 & 1.07 & 1.03 \\ \hline
\end{tabular}
\caption{Polish Dataset}
\label{tab:polish_kl_dv}
\end{subtable}%
\hfill
\begin{subtable}{0.36\linewidth}
\centering
\begin{tabular}{r|rrrrr}
\hline
\textbf{Variable} & \textbf{S} & \textbf{P} & \textbf{D} & \textbf{CP} & \textbf{CC} \\ \hline
age & 1.00 & 0.98 & 0.99 & 1.05 & 0.99 \\
workclass & 1.00 & 1.11 & 1.00 & 1.03 & 1.00 \\
education & 1.00 & 1.03 & 1.01 & 1.02 & 1.00 \\
marital.status & 1.00 & 1.27 & 1.01 & 1.03 & 1.01 \\
occupation & 1.00 & 1.22 & 1.04 & 0.99 & 1.01 \\
relationship & 1.00 & 1.36 & 0.97 & 0.99 & 0.97 \\
race & 1.00 & 1.51 & 1.05 & 1.02 & 0.98 \\
sex & 1.00 & 1.46 & 1.03 & 1.03 & 0.95 \\
capital.gain & 1.00 & 24.81 & 1.03 & 1.18 & 1.00 \\
capital.loss & 1.00 & 22.35 & 1.05 & 1.22 & 1.00 \\
hours.per.week & 1.00 & 1.44 & 1.05 & 1.14 & 1.03 \\
native.country & 1.00 & 2.03 & 1.11 & 1.03 & 1.00 \\
income & 1.00 & 62.92 & 1.15 & 1.07 & 1.01 \\ \hline
Average & 1.00 & 9.50 & 1.04 & 1.06 & 1.00 \\ \hline
\end{tabular}%
\caption{Adult Dataset}
\label{tab:adult_kl_dv}
\end{subtable}%
\hfill
\begin{subtable}{0.36\linewidth}
\centering
\begin{tabular}{r|rrrrr}
\hline
\textbf{Variable} & \textbf{S} & \textbf{P} & \textbf{D} & \textbf{CP} & \textbf{CC} \\ \hline
Int\_Dist & 1.00 & 0.99 & 0.98 & 0.97 & 1.00 \\
Up\_Marg & 1.00 & 1.04 & 1.01 & 0.98 & 1.00 \\
Lo\_Marg & 1.00 & 1.43 & 0.98 & 0.97 & 0.98 \\
Exploit & 1.00 & 1.08 & 1.07 & 1.02 & 1.44 \\
Row\_Num & 1.00 & 8.69 & 1.07 & 1.02 & 1.09 \\
Mod\_Ratio & 1.00 & 1.51 & 1.09 & 1.00 & 1.03 \\
Int\_Spac & 1.00 & 1.28 & 1.03 & 1.07 & 1.04 \\
Weight & 1.00 & 1.33 & 1.18 & 1.13 & 1.10 \\
Peak\_Num & 1.00 & 6.78 & 1.18 & 1.26 & 1.15 \\
MR/IS & 1.00 & 17.85 & 1.07 & 1.95 & 1.04 \\
Class & 1.00 & 34.64 & 1.26 & 1.02 & 1.03 \\ \hline
Average & 1.00 & 6.96 & 1.08 & 1.13 & 1.08 \\ \hline
\end{tabular}
\caption{Avila Dataset}
\label{tab:avila_kl_dv}
\end{subtable}
}
\end{table*}

==> imputation.tex <==
% \subsection{Data Synthesis}
% The goal of
% In statistics, imputation is the process of replacing missing data with substitute values drawn from similar records. It was originally developed for solving the problem of missing values in surveys. With singular imputation methods single values are used to impute missing values which introduces a level of uncertainty regarding which values to impute. To be able to assess the uncertainty introduced while retaining the advantages of the imputation process, Rubin \cite{rubin1987multiple} developed an approach called multiple imputation. 

% Multiple imputation replaces each missing value with multiple values instead of one single value, generated based on a probability distribution for new values given the observed data. The resulting $m\;(where\;m>1)$ datasets are then treated as multiple datasets. Each of the  $m$ imputed datasets is first analyzed using standard statistical methods developed for complete data. Then the resulting $m$ analysis are consolidated to produce intended estimates with proper reflection of the imputation uncertainty.  

% %To make an inference, the results from these datasets are consolidated into one result either by using any standard statistical methods (e.g. mean, variance, or confidence interval) or by combining simulations from each separate model

% In the year 1993 Rubin \cite{rubin1993statistical} first coined the idea of using multiple imputation to generate fully synthetic datasets. The basic idea proposed by him is to treat the population not selected in a sample as missing data and then use multiple imputation to create synthetic datasets. Such synthetic datasets then can then be used to draw conclusions of relationships between features that would be true for the original data.

% For multiple imputation, there are two general approaches that have emerged over the years to generate draws from probability distribution $P(Y_{new}|Y_{obs})$ (where $Y_{new}$ represents the missing values or values to be imputed): joint modeling approach and fully conditional specification (FCS) approach \cite{Drechsler2011}. With the FCS approach variables are replaced in a specific order whereas with the joint modeling approach multiple variables are replaced together.

% The joint modeling approach is performed under the assumption that the data follows a specific distribution (e.g.  a multivariate normal distribution). However, FCS approach does not make any assumptions for the joint distribution of the dataset, rather lets each variable to follow its own distribution that are conditioned on other variables such as: $P(Y_j|Y_{-j},\theta_j)$ where $j$ refers to a specific variable/column, $-j$ refers to a subset of columns/variables excluding $j$ from which $P(Y_{new}|Y_{obs})$ can be drawn. Based on which variables to include in $-j$, there are two approaches to generate synthetic values. One approach is to include variables not yet synthesized in $-j$ and use a mix of synthesized values and originals when new values are drawn. Another approach is to only use variables that have been synthesized for drawing new values. The latter one has on an average a small negative effect on the utility and privacy, however it greatly reduces the computation time \cite{Caiola2010}.

% \noindent\textbf{Imputation Order.} For the joint modeling  approach, the values in each record is generated at once whereas for FCS a particular order needs to be selected to impute the variables. The order that seems most logical is usually chosen. There are other approaches also for choosing the order. For instance, in \cite{Reiter2005} the order was chosen from smallest to largest number of values that needed to be replaced and it was possible since only some specific values were replaced. However, to replace all values, the order needs to be chosen based on the relations between the variables and also the computational complexity.

% \noindent\textbf{Simple \& Selective Imputation.} For the FCS pproach, it is possible to select which variables to use for the imputation of each variable. Being selective about the variables during imputation can have some positive as well as some negative impacts. For instance, choosing a subset of variables for imputation can reduce the computation time and also can preserve the relationships between variables that are most essential. However, the downside is that the correlations that are not chosen can get lost and to know which relationships to preserve is also not straightforward. Thus, choosing all variables for each imputation is far more simple procedure.

% Depending on which variables to choose for generating missing values, imputation can be of two types, we term those as Simple imputation and Selective imputation.  The Simple approach is to use every other variable in the imputation while Selective instead only uses a subset of the variables for the imputation.

% \noindent\textbf{Proper \& Non-proper Imputation.} Depending on whether you sample from original dataset or not while generating imputation models, imputation can be of two types, Proper imputation and Non-Proper imputation. When imputation models are generated the Proper methodology samples records from the original dataset to create the models while Non-Proper just uses all the records from the original dataset without any sampling.

==> metrics.tex <==
\section{Methods to Determine Utility}
%There exists several methods in the literature for estimating the utility provided by synthetic data compared to the original data.

The existing works on synthetic data use different metrics to estimate the utility provided by such data. However, there is no such metric that can individually capture all the different aspects of utility with regards to synthetic data. Hence, a combination of different metrics is needed to compare the utility provided by synthetic data and the original data. We found four different methods for estimating the utility of synthetic data which are: checking how well synthetic values conform to original distributions \cite{Hawala2008}, comparison of average estimate together with variance of synthetic data with the original data to see if inferences still hold for synthetic data\cite{Reiter2002}, comparison of specific inferences in the original data and in the synthetic data \cite{Karr2006}, and Kullback-Leibler (KL) divergence \cite{Dandekar2018} for global utility measures.

\noindent\textbf{Synthetic Values Conform to Original Distributions.} This is a fairly simple utility test which checks whether the synthetic values have similar distributions as the original values. One way to achieve that is to compare the mean and variance of the variables in the synthetic data and the original data. Another method is to check how many of the synthetic values are within the $95\%$ confidence interval of the original data. The idea here is that if the synthetic data matches well with the original data then the synthetic values should lay $95$ \% of the time within the confidence interval of original values. These kind of comparisons only shows how each variable's univariate distributions compare, however, they do not say anything about how well the correlations between the variables are preserved.

\noindent\textbf{Compare Average Estimator and Variance.} 
\label{CAEV}
This methodology has been developed for multiple imputation with the Little method in \cite{Reiter2003} and has been used in further studies such as \cite{Reiter2005} and \cite{Drechsler2018}. An estimator $q$ is a type of scalar function that acts on the synthetic data as an estimate of the true value $Q$ that one would get from the original data. Since there are $m$ number of different datasets one gets $m$ number of estimates of $Q$, $q_i$ which provides an average estimator
\[\bar{q}_m = \sum_{i=1}^m q_i / m\]
and an average variance of the estimator
\[\bar{v}_m = \sum_{i=1}^m v_i / m\]
Those two together with
\[b_m = \sum_{i=1}^m (q_i - \bar{q}_m)^2 / (m-1)\]
and
\[T_p = \bar{v}_m + b_m m^{-1}\]
can be used to get valid inferences for $Q$ and the variance of $Q$ where $\bar{q}_m$ is used to estimate $Q$ and $T_p$ is used to estimate the variance of $Q$. %Inferences are then based on $\bar{q}_m$, $T_p$ and a student's t reference test.

There is also an alternative variance estimator:
\[T_s = (1 + \frac{1}{m})\bar{v}_m\]
which also functions when there is only one synthetic dataset ($m = 1$) but has some limitations on when it can be used \cite{Drechsler2018}. 

\noindent\textbf{Compare Specific Inferences in Original and Synthetic Datasets.} In paper \cite{Karr2006}, two utility measuring frameworks are discussed. One is based on a global measure of utility and compares the distributions of the variables in the original and the synthetic datasets while the other method looks at specific inferences in the original and the synthetic data and compare the two. The second method might at first glance seem inadequate, only providing an idea of how well the data works for the specific inferences checked while not knowing how well the others are. The argument for that methodology however is that there are many datasets for which one already knows beforehand what inferences are important or are going to be used and so checking those are adequate or even sufficient to determine if the synthetic data are going to be useful or not \cite{Drechsler2008}. Another consideration is how likely it is that a synthetic dataset that has shown good utility for a diverse set of inferences would just happen to only be good for these but not for others not tested. This paper \cite{Karr2006} does argue also that good practise would be to check specific inferences and some global measure to ensure that the data is both good in a general sense and in at least some specific cases too.

\noindent\textbf{Kullback-Leibler Divergence.} Kullback-Leibler Divergence is used to measure how close two probability distributions are, based on information entropy and is what is known as a "global measure of data utility"\cite{Woo2009}. This report \cite{Dandekar2018} used normalized KL divergence score to derive a metric to compare the methods. This is somewhat similar to the first method to verify if the synthetic values conform to the original distributions but instead of checking means and variances the distributions themselves are compared. KL divergence for discrete distributions are defined as follows:

\[D_{KL}(P|Q) = \sum_{x \in X} P(x) log \left(\frac{P(x)}{Q(x)} \right) \]

$P$ and $Q$ is then the distribution of a variable from the original dataset and the distribution of the same variable from a synthetic dataset though it does not matter which is which as long as it is consistent. It is also possible to calculate for both alternatives and then use the average of the two. For categorical variables, X is just the different values while for the numerical variables, X is a quantization with the upper and lower bounds being the largest and smallest value from the original and the synthetic datasets with a step-size of suitable magnitude.

Multivariate distributions are also possible to compare which means that relations between variables can also be compared. Calculating the KL divergence score can be complicated depending on the distributions so a Markov Chain Monte Carlo approximation is often used instead, especially for multivariate distributions.

\subsection{Utility Metrics}
To measure or estimate utility, in this work, we will use a combination of mean point estimators, regression fit coefficient estimation and KL-divergence scores. We will calculate Confidence Interval (CI) for the mean point estimators and the regression fits coefficients estimations and the real coefficients from the original data. We will then create Confidence Interval Overlaps (CIO) according to this formula:
%\centering\scalebox{0.9}{$ CIO = max(0.5 \cdot \left(\frac{min(U_o,U_s)-max(L_o,L_s)}{U_o-L_s}+\frac{min(U_o,U_s)-max(L_o,L_s)}{U_s-L_o}\right),0)$}\\
\begin{equation}
\begin{small}
    \scalebox{0.9}{$CIO = max(0.5 \cdot \left(\frac{min(U_o,U_s)-max(L_o,L_s)}{U_o-L_s}+\frac{min(U_o,U_s)-max(L_o,L_s)}{U_s-L_o}\right),0)$}
\end{small}
\end{equation}
Where $L$ and $U$ are the lower and upper bounds for the synthetic ($s$) and original ($o$) CI. We have a lower bound on $CIO$ because it can otherwise grow to large negative numbers if the CI do not overlap. We will check the average utility for each synthesizer to get an idea about how well each synthesizer performs.
For the KL-divergence, we will measure the scores for each individual released dataset and then average them to get one KL-divergence score.

\noindent{\textbf{What is a good utility for Synthetic Data.}}
Given the utility metrics, we need to define the criteria for good or acceptable utility for synthetic data. As mentioned previously, utility metrics mean point estimators and regression fitting can be compared with Confidence Interval Overlaps (CIO). However, there are no obvious intervals where the CIO is good or bad. There are some previous works \cite{Reiter2005b}) that try to define some specific criteria. According to the literature, for the overlap everything over $90$\% is considered good, between $90$ and $50$ is considered as bad and below $50$ is useless. Even though $90$\% may seem too stringent at first there are arguments behind it. The above $90$\% overlap guarantees that the synthetic coefficient is both close to the original (at least reasonably close based on the variance) and that the confidence intervals are also closely matching in size.

In the case of overlap further away from $90$, there can be situations where either the confidence intervals match but they are far apart or the opposite scenario where the intervals are close together but they do not match or are very dissimilar. There can also be extreme cases where one confidence interval may entirely reside in one side of the other interval. Below $50$ means that the coefficients do not reside in each others confidence intervals and can be discarded immediately. Since for the synthetic data the more the number of CI overlaps above $90$\% the better the utility, it is more appropriate to calculate the Average Percentage of CI overlaps (APO) above $90$ instead of calculating the average CI overlaps. So, in this work, we calculate APO above $90$\%  to evaluate the utility of the synthetic data.

In the case of KL-divergence, it is hard to determine if a result is good on its own since the value only indicates how close two distributions are. The value does not say anything how well the synthetic datasets follows the original. However, the values can be used to compare among the different alternative methods to find out which method produces datasets that follow the original distributions most closely.


==> sysnthesizers.tex <==
% \section{Methods for Synthetic Data Generation}
% There are several methods developed over the years for generating synthetic data using multiple imputation. Parametric and Decision Trees are the two most widely used methods. These methods are based FCS approach. Saturated model is also a well known method which is based on joint modelling approach.   

% \subsection{Parametric}
% In parametric method, the first variable is chosen together with a suitable regression model. A subset of the variables are then fitted to it and beta-coefficients ($\beta$) and variances ($\sigma^2$) are estimated. Those are then used together with $Y_{-j}$ in some distribution like: $N(\beta Y_{-j}, \sigma^2)$ to draw synthetic values from. When that is done the second variable is picked and a regression is made to fit the other variables to it but this time the new synthetic values are used instead. The parametric method uses different kind of regression models depending on what type of data values are meant to be synthesized with linear regression used for numerical variables and logistic regression used for categorical variables.

% \subsection{Decision Trees}
% Decision Trees or as they are commonly referred to in machine learning Classification and Regression Trees (Cart) is a non-parametric alternative to the Parametric methodology \cite{Nowok2017}. Using decision trees to generate synthetic data was introduced in \cite{Reiter2005} and was based on previous work on replacing missing values, just like Parametric. A decision tree can be used to represent a multivariate conditional distribution so instead of trying to fit a regression model on the variable, a decision tree is created for the imputed variable which is split on the subset of variables.

% A decision tree can be visualized as a flow chart where at each decision, the tree is split i.e. a test is made against the value of some variable/s for which path to take. After going through the tests down the tree, one ends up at a leaf which holds some number of values for the variable we are imputing. To create such a tree, it starts with all values for the variable as one leaf each with splits based on the values of the other variables. The tree is then pruned so that some leaves are combined and the remaining leaves hold a number of different values. After going down the tree to one leaf, one value is sampled from the values within the leaf.

% \subsection{Saturated Model}
% The Saturated Model approach works by fitting a model that perfectly reproduces the data, to a cross-tabulated table of all the categorical variables \cite{Lee2009, Catall}. Certain combinations in the cross-tabulation can be manually excluded from being used for imputation by giving them a zero probability in the multinomial distribution. Synthetic values are then imputed by sampling from the multinomial distribution where the parameters come from the probabilities of each variable combination. Since this method only works with categorical variables, a parametric method or decision tree is needed in combination for the numerical variables. An interesting difference between Saturated Model and the two other approaches is that Saturated Model is strictly a joint modelling based approach while Parametric and Decision Trees are mostly FCS based approaches.

% \input{figures_tables/tb_naming_convention}

% \subsection{Synthesizer Software}
% A program called synthpop \cite{Nowok2016} for the R language provides a framework for generating synthetic data based on the multiple imputation methodology. It includes different methods for Parametric and two implementations for Decision Trees. It also has a saturated model implementation for categorical variable termed as \emph{Catall}.  In this work, we use the default parametric method as the Parametric synthesizer, the Cart implementation as the Decision Tree synthesizer, a combination of Catall and Predictive Mean Matching (PMM) for the Saturated Model with Parametric, and Catall and Cart for the Saturated Model with Decision Trees. We will refer to these four as Standard Parametric (SAP), Cart, Catall with PMM (CAP), and Catall with Cart (CAC) as shown in Table \ref{table:naming_convention}. We also create the fifth synthesizer: Sample, which just imputes the synthetic variables by sampling from the original dataset without using any relationships between the variables. Thus, sample should provide good results for the utility tests that only check the univariate distributions but not the relationships between variables.

